The Overfocusing Bias of Convolutional Neural Networks: A Saliency-Guided Regularization Approach

Despite transformers being considered as the new standard in computer vision, convolutional neural networks (CNNs) still outperform them in low-data regimes. Nonetheless, CNNs often make decisions based on narrow, specific regions of input images, especially when training data is limited. This behavior can severely compromise the model's generalization capabilities, making it disproportionately dependent on certain features that might not represent the broader context of images. While the conditions leading to this phenomenon remain elusive, the primary intent of this article is to shed light on this observed behavior of neural networks. Our research endeavors to prioritize comprehensive insight and to outline an initial response to this phenomenon. In line with this, we introduce Saliency Guided Dropout (SGDrop), a pioneering regularization approach tailored to address this specific issue. SGDrop utilizes attribution methods on the feature map to identify and then reduce the influence of the most salient features during training. This process encourages the network to diversify its attention and not focus solely on specific standout areas. Our experiments across several visual classification benchmarks validate SGDrop's role in enhancing generalization. Significantly, models incorporating SGDrop display more expansive attributions and neural activity, offering a more comprehensive view of input images in contrast to their traditionally trained counterparts.

==> ARXIV/sections/0_abstract.tex <==

\begin{abstract}
Deep neural networks, especially in situations with sparse training data, often make decisions based on narrow, specific regions of input images. This behavior can severely compromise the model's generalization capabilities, making it disproportionately dependent on certain features that might not represent the broader context of images.
While the conditions leading to this phenomenon remain elusive, the primary intent of this article is to shed light on this observed behavior of neural networks. Rather than striving for the pinnacle of performance, our focus is on deepening understanding and offering an initial solution to the challenge. In line with this, we introduce the Saliency Guided Dropout (SGDO), a pioneering regularization approach tailored to address this specific issue.
SGDO utilizes attribution methods on the feature map to identify and then reduce the influence of the most salient features during training. This process encourages the network to diversify its attention and not focus solely on specific standout areas. Our experiments across X visual classification benchmarks validate SGDO's role in enhancing generalization. Significantly, models incorporating SGDO display more expansive attributions and neural activity, offering a more comprehensive view of input images in contrast to their traditionally trained counterparts.
%This paper provides insight into the challenges of localized focus in neural networks and introduces SGDO as a promising step towards addressing this issue.
\keywords{First keyword \and Second keyword \and Third keyword}
\end{abstract}

==> ARXIV/sections/3_background.tex <==

\section{Background}
\label{sec:Background}
We consider the supervised classification problem, which entails discovering a function $f$ within a hypothesis space $\mathcal{H}$ that maps an input feature space $\mathcal{X}$ to a discrete set of output labels $\mathcal{C}$.
For the underlying distribution $p(x,c)$ on input-class pairs $(x,c) \in \mathcal{X} \times \mathcal{C}$, $f$ should capture the dependency of $c$ on $x$.
Note that we set ourselves in a fairly general framework, where an element $x\in \mathcal{X}$ can be an image, but also a map of features on a image, or even a vector of values in $\mathbb{R}^n$. 
We adopt the classical reformulation where one searches for $f$ as a $\mathcal{X} \rightarrow \mathbb{R}^{|\mathcal{C}|}$ mapping, predicting probabilities of each class $c\in\mathcal{C}$. 
The most adequate $f$ is the one which minimizes the empirical risk $\frac{1}{n} \sum_{i=1}^{n} \ell(f(x_i),y_i)$, relying on a finite sample of input-label pairs ${(x_i,y_i)}_{i=1}^n$ drawn independently from $p$ \cite{vapnik1991principles}. 
%The objective is to minimize the expected risk function $\mathcal{R}(f)=\mathbb{E}{(x,y)\sim p}[\mathcal{L}(f(x),y)]$, with $\mathcal{L}(\hat{y},y)$ being the loss function that quantifies the classification error.
%In practice, we approximate $\mathcal{R}(f)$ with the empirical risk \cite{vapnik1991principles}$ \mathcal{R}{emp}(f) = \frac{1}{n} \sum_{i=1}^{n} \mathcal{L}(f(x_i),y_i)$, relying on a finite sample of image-label pairs ${(x_i,y_i)}_{i=1}^n$ from the probability distribution $p$.
Throughout the remainder of this paper, we define $\mathcal{H}$ as the space of neural network functions with parameters $\theta$. 
We define an attribution map for a network $f \in \mathcal{H}$ as a function $\mathcal{A}_f : \mathcal{X} \times \mathcal{Y} \to \mathbb{R}^d$ that quantifies the contribution of each feature in $\mathcal{X}$ to the prediction for a target class $c \in \mathcal{Y}$ by $f$. Formally, for an input image $x \in \mathcal{X}$ and class label $c \in \mathcal{Y}$, the attribution map is given by:
\begin{equation}
\mathcal{A}_f(x, c) = \text{attrib}(x, c; \theta),
\end{equation}
where $\text{attrib}$ is a method-specific operator that determines the relevance of each feature in $x$ for the classification of $c$.





==> ARXIV/sections/9_rebuttal.tex <==
\section{Reviewer ZU7K}
    \begin{itemize}
        \item Refaire la figure 1 avec les accuracy train et test -> David XP, Mehdi figures
        \item Comparaison avec les autres methodes exitation backprop, dropout, cut-out, sur pixels -> David
        \item Transformers -> bonne réponse réponse + citations autres papier? -> Hugo 
        \item Réponse sur data-augmentation -> David 
        \item Répondre sur l'hyperparamètre/ essayer de comprendre le phénomène. NA
        \item Implémenter SGQN, BlockDrop, ... -> Mehdi
    \end{itemize}

Hugo: Keep this link here: https://openaccess.thecvf.com/content/ICCV2023/papers/Psomas_Keep_It_SimPool_Who_Said_Supervised_Transformers_Suffer_from_Attention_ICCV_2023_paper.pdf (Figure 1: CLS token generates an attention map that overfocuses on a given region)

\section{rtLH}
\begin{itemize}
    \item Réponse structure du papier -> Manu?
    \item Réponse computation graph + mention du code + shéma -> David
    \item Convnext -> Hugo satélitte DAvid Imagenette/woof
    \item Réponse transformer et essayer l'experience 1 sur le transformer et le token CLS -> Mehdi
    \item Transfer sur RSICD -> Hugo
    \item general comment sur work in progress + novelty -> Manu?
\end{itemize}

A) Experiments on ConvNeXt
\begin{table*}[!ht]
  \centering
  \begin{tabular}{@{}llccccc@{}}
    \toprule
    Network                  & Method              & Imagenette       & Imagewoof   & RSICD            & RESISC45         & PatternNet       \\
    \midrule
    \multirow{4}{3em}{ConvNeXt} & Baseline                   &  &  & 48.03 & 67.01 & 96.22 \\
                                & Dropout                    &  &  & 53.98 & 72.09 & 96.98 \\
                                & Excitation Dropout         &  &  &   -   &   -   &   -   \\
                                & SGDrop                     &  &  & 55.81 & 73.46 & 97.51 \\
                                & SGDrop (curriculum $\rho$) &  &  & 52.70 & 74.58 & 97.15 \\
    \bottomrule
  \end{tabular}
  \caption{ConvNeXt performance.}
  \label{tab:Comparison_with_methods_across_datasets}
\end{table*}
Hugo: SGDrop improves over the other methods! :)
Interesting: Excitation dropout faces some CUDA issues after ~3 epochs and trainings are not finished. This behavior has been reported uniquely in ConvNeXt so far...

B) Transfer learning experiments (10 epochs)
Pretraining models on RESISC45 (30k images) using VGG (because we have nice results) using these configs: Baseline, Dropout, Excitation Dropout, SGDrop and SGDrop (curriculum $\rho$)
Respective accuracies: 64.58, 66.82, 66.62, 83.36, 84.13.
Paths:
Baseline: /opt/hugo/Projects/deel/AtDrop/results/mlruns/600589900902234230/e6e5460da3424d0ab9e98e998c71f82b/saved_models/trained_model_epoch_4.bin
Dropout: /opt/hugo/Projects/deel/AtDrop/results/mlruns/600589900902234230/80049e57beb24547b7ea4658e24065a8/saved_models/trained_model_epoch_60.bin
Excitation: /opt/hugo/Projects/deel/AtDrop/results/mlruns/600589900902234230/64f30e87fa104a4dac97adc5fe7da0db/saved_models/trained_model_epoch_6.bin
SGDrop: /opt/hugo/Projects/deel/AtDrop/results/mlruns/600589900902234230/b8bf6ca54abf49cebc63103b56ec260e/saved_models/trained_model_epoch_79.bin
SGDrop curriculum: /opt/hugo/Projects/deel/AtDrop/results/mlruns/600589900902234230/39f0159c8ae140a0af17dca9a3a4d5ac/saved_models/trained_model_epoch_78.bin
-> Interesting: See the best epoch per method
-> These pretrained models are used to fine-tune on RSICD (8k images)

-> 10 epochs
-> The classification layer is the only trainable layer
\begin{table}
  \centering
  \begin{tabular}{@{}lcc@{}}
    \toprule
    Method                     & RESISC45  & RSICD (from RESISC45)\\
    \midrule
    Baseline                   & 64.58 & 63.68 \\
    Dropout                    & 66.82 & 65.60 \\
    Excitation Dropout         & 66.62 & 64.50 \\
    SGDrop                     & 83.36 & 69.99 \\
    SGDrop (curriculum $\rho$) & 84.13 & 70.27 \\
    \bottomrule
  \end{tabular}
  \caption{Transfer learning RESISC45 $\rightarrow$ RSICD. Accuracy reported on the test split.}
  \label{tab:Transfer_learning}
\end{table}
Hugo: Nice, good results!!

\section{rT2z}
\begin{itemize}
    \item répondre sur les comparaisons avec saliency guided -> Après XP Mehdi
    \item dire que a première weakness et une strenght? -> David
    \item demander explicitement de rajouter un point
\end{itemize}

\section{réponse générale}
\begin{itemize}
    \item Rappeler la partie transformer
    \item Comparaison avec état de l'art
\end{itemize}
